Grokking at the Edge of Numerical Stability

Grokking, the sudden generalization that occurs after prolonged overfitting, is a surprising phenomenon challenging our understanding of deep learning. Although significant progress has been made in understanding grokking, the reasons behind the delayed generalization and its dependence on regularization remain unclear. In this work, we argue that without regularization, grokking tasks push models to the edge of numerical stability, introducing floating point errors in the Softmax function, which we refer to as Softmax Collapse (SC). We demonstrate that SC prevents grokking and that mitigating SC enables grokking without regularization. Investigating the root cause of SC, we find that beyond the point of overfitting, the gradients strongly align with what we call the na\"ive loss minimization (NLM) direction. This component of the gradient does not alter the model's predictions but decreases the loss by scaling the logits, typically by scaling the weights along their current direction. We show that this scaling of the logits explains the delay in generalization characteristic of grokking and eventually leads to SC, halting further learning. To validate our hypotheses, we introduce two key contributions that address the challenges in grokking tasks: StableMax, a new activation function that prevents SC and enables grokking without regularization, and $\perp$Grad, a training algorithm that promotes quick generalization in grokking tasks by preventing NLM altogether. These contributions provide new insights into grokking, elucidating its delayed generalization, reliance on regularization, and the effectiveness of existing grokking-inducing methods. Code for this paper is available at https://github.com/LucasPrietoAl/grokking-at-the-edge-of-numerical-stability.

==> outline_drafts.tex <==
\begin{itemize}
    \item Intro: bservation that actually ``something'' is happening in no-regularization training, suspiciously exactly when WD leads to grokking.
    \item This is softmax collapse (SC)
    \item SC is prevalent: Every time we see grokking, SC is \textit{suspiciously} always there.
    \begin{itemize}
        \item WD: Removing WD leads to SC
        \item L1 regularization
        \item Dataset size: Decreasing dataset size leads to SC
        \item 1-layer MSE: Adding two layers leads to SC (p.s. name has to change for this)
    \end{itemize}
    \item Preventing SC through other interventions creates grokking (with varying success, given physical limitations)
    \begin{itemize}
        \item Float64
        \item Taylor approximation
        \item Stable sum
    \end{itemize}
    \item WD is great, but not for the reasons you think. 
        \begin{itemize}
            \item WD is not great because of its inductive bias, but possibly because it does not have a lot of inductive bias.
            \item It's not like WD has no useful inductive biases at all: e.g. implicit learning rate increase.
        \end{itemize}
    \item Implications for general ML
\end{itemize}

Points to keep in mind:
- Defer margin maximization and difficulty comparison between original task vs. memorization to later in writing.
